Dynamic Link Network Emulation: a Model-based Design

This paper presents the design and architecture of a network emulator whose links' parameters (such as delay and bandwidth) vary at different time instances. The emulator can thus be used in order to test and evaluate novel solutions for such networks, before their final deployment. To achieve this goal, different existing technologies are carefully combined to emulate link dynamicity, automatic traffic generation, and overall network device emulation. The emulator takes as an input a formal model of the network to emulate and configures all required software to execute live software instances of the desired network components, in the requested topology. We devote our study to the so-called dynamic link networks, with potentially asymmetric links. Since emulating asymmetric dynamic links is far from trivial (even with the existing state-of-the-art tools), we provide a detailed design architecture that allows this. As a case study, a satellite network emulation is presented. Experimental results show the precision of our dynamic assignments and the overall flexibility of the proposed solution.

==> figures/dama_algorithm.tex <==
\begin{algorithm}[!htb]
%\begin{algorithm}[H]
\small
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKw{KwBy}{b}\SetKw{Goto}{go to}

    \Input{A network topology $G=(V,E)$, the cluster bandwidth $B$, the CIR, MIR and demands per link $c:E\to \mathds{Z}_{\geq0}$, $m:E\to \mathds{Z}_{\geq0}$, and $d:E\to \mathds{Z}_{\geq0}$, respectively, and $u\in \mathds{Z}_{\geq1}$ an allocation unit, such that $u<B$ and $\forall e\in E\;u\leq c(e)$}
    \Output{A bandwidth assignation $b:E\to \mathds{Z}_{\geq0}$}
    \textbf{Step 0:} Set $b(e)\leftarrow 0\;\;\forall e\in E\;$ and Set $R\leftarrow0$
    %\tcp{$R$ a variable to check the remaining resources requested}
    \textbf{Step 1:} \ForEach{$e\in E$}
    {
        \If{$B \geq c(e)$}
        {
            Set $b(e)\leftarrow min \{max\{u, d(e)\}, c(e)\}$
            \tcp{Assign the bandwidth either the demanded amount, the minimal allocation unit or its CIR}
            Set $d(e)\leftarrow max\{u, d(e)\} - b(e)$
            %\tcp{Re-adjust the demand for further processing}
            Set $R\leftarrow R + d(e)$\;
            Set $B\leftarrow B - b(e)$\;
        }
    }
    \textbf{Step 2:} \If{$B\geq R$}
    {
        \ForEach{$e \in E$}
        {
        % Erick : Update in -> $b(e)\leftarrow b(e) + min \{b(e)+d(e), m(e)\}$ ; adding b(e) increase value. 
            Set $b(e)\leftarrow min \{b(e)+d(e), m(e)\}$
            \tcp{Assign the bandwidth either the demanded amount or its MIR}
        }
        \Goto \textbf{Step 4}\;
    }
    \textbf{Step 3:} \While {$B > 0$ and $R > 0$}
    {
        Set $R\leftarrow 0$\;
        \ForEach{$e \in E$}
        {
            Let $a\leftarrow min \{d(e), u, B\}$
            
            \tcp{$a$ is a bandwidth addition for the link, either the remainder demanded amount, the allocation unit, or the rest of the available bandwidth}
            \If{$(b(e)+ a) \leq m(e)$}
            {R
                Set $b(e)\leftarrow b(e) + a$
                \tcp{Assign the bandwidth either the demanded amount the allocation unit}
                Set $d(e)\leftarrow d(e) - a$
                %\tcp{Re-adjust the demand for further processing}
                Set $B\leftarrow B - a$\;
            }
            \Else 
            {
                Set $d(e)\leftarrow 0$
                \tcp{No more bandwidth can be assigned to the demand due to its MIR}
            }
            Set $R\leftarrow R + d(e)$\;
            \If{$B = 0$}
            {
                \Goto \textbf{Step 4}\;
            }
        }
    }
    \textbf{Step 4:} \Return{$b$}
    \caption{DAMA algorithm}\label{algo:dama}
\end{algorithm}

==> figures/graphs/band_graph_constant.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
    ymax=10, 
    ymin=0,
	ylabel={Bandwidth (Mbps)},
	xlabel={Time (ms)},
	legend style={at={(0.02,0.98)}, 
	anchor=north west},
]
\addplot[smooth,blue] coordinates
{

(	1	,	4   )
(	2	,	4	)
(	3	,	4	)
(	4	,	4	)
(	5	,	4	)
(	6	,	4	)
(	7	,	4	)
(	8	,	4	)
(	9	,	4	)
(	10	,	4	)
(	11	,	4	)
(	12	,	4	)
(	13	,	4	)
(	14	,	4	)
(	15	,	4	)
(	16	,	4	)
(	17	,	4	)
(	18	,	4	)
(	19	,	4	)
(	20	,	4	)
(	21	,	4	)
(	22	,	4	)
(	23	,	4	)
(	24	,	4	)
(	25	,	4	)
(	26	,	4	)
(	27	,	4	)
(	28	,	4	)
(	29	,	4	)
(	30	,	4	)
(	31	,	4	)
(	32	,	4	)
(	33	,	4	)
(	34	,	4	)
(	35	,	4	)
(	36	,	4	)
(	37	,	4	)
(	38	,	4	)
(	39	,	4	)
(	40	,	4	)
(	41	,	4	)
(	42	,	4	)
(	43	,	4	)
(	44	,	4	)
(	45	,	4	)
(	46	,	4	)
(	47	,	4	)
(	48	,	4	)
(	49	,	4	)
(	50	,	4	)
(	51	,	4	)
(	52	,	4	)
(	53	,	4	)
(	54	,	4	)
(	55	,	4	)
(	56	,	4	)
(	57	,	4	)
(	58	,	4	)
(	59	,	4	)
(	60	,	4	)
(	61	,	4	)
(	62	,	4	)
(	63	,	4	)
(	64	,	4	)
(	65	,	4	)
(	66	,	4	)
(	67	,	4	)
(	68	,	4	)
(	69	,	4	)
(	70	,	4	)
(	71	,	4	)
(	72	,	4	)
(	73	,	4	)
(	74	,	4	)
(	75	,	4	)
(	76	,	4	)
(	77	,	4	)
(	78	,	4	)
(	79	,	4	)
(	80	,	4	)
(	81	,	4	)
(	82	,	4	)
(	83	,	4	)
(	84	,	4	)
(	85	,	4	)
(	86	,	4	)
(	87	,	4	)
(	88	,	4	)
(	89	,	4	)
(	90	,	4	)
(	91	,	4	)
(	92	,	4	)
(	93	,	4	)
(	94	,	4	)
(	95	,	4	)
(	96	,	4	)
(	97	,	4	)
(	98	,	4	)
(	99	,	4	)
(	100	,	4	)
(	101	,	4	)
(	102	,	4	)
(	103	,	4	)
(	104	,	4	)
(	105	,	4	)
(	106	,	4	)
(	107	,	4	)
(	108	,	4	)
(	109	,	4	)
(	110	,	4	)
(	111	,	4	)
(	112	,	4	)
(	113	,	4	)
(	114	,	4	)
(	115	,	4	)
(	116	,	4	)
(	117	,	4	)
(	118	,	4	)
(	119	,	4	)
(	120	,	4   )
 

};\addlegendentry{Demand}


%\addplot[smooth,mark=*,red] coordinates
\addplot[smooth,red] coordinates
{

(1.00 , 3.76)
(2.00 , 3.72)
(3.00 , 3.74)
(4.00 , 3.73)
(5.00 , 3.72)
(6.00 , 3.74)
(7.00 , 3.65)
(8.01 , 3.44)
(9.01 , 2.33)
(10.00 , 2.29)
(11.00 , 2.97)
(12.00 , 3.06)
(13.00 , 3.38)
(14.00 , 3.63)
(15.00 , 2.65)
(16.00 , 3.11)
(17.00 , 3.21)
(18.00 , 3.62)
(19.00 , 3.59)
(20.00 , 3.73)
(21.00 , 3.74)
(22.00 , 3.74)
(23.00 , 3.69)
(24.00 , 3.72)
(25.00 , 3.74)
(26.00 , 3.72)
(27.00 , 3.73)
(28.00 , 3.74)
(29.00 , 3.74)
(30.00 , 3.74)
(31.00 , 3.72)
(32.00 , 3.70)
(33.00 , 3.73)
(34.00 , 3.74)
(35.00 , 3.74)
(36.00 , 3.74)
(37.00 , 3.76)
(38.00 , 3.74)
(39.00 , 3.68)
(40.00 , 3.74)
(41.00 , 3.74)
(42.00 , 3.74)
(43.00 , 3.74)
(44.00 , 3.74)
(45.00 , 3.75)
(46.00 , 3.74)
(47.00 , 3.74)
(48.00 , 3.74)
(49.00 , 3.74)
(50.00 , 3.73)
(51.00 , 3.76)
(52.00 , 3.74)
(53.00 , 3.74)
(54.00 , 3.74)
(55.00 , 3.74)
(56.00 , 3.75)
(57.00 , 3.74)
(58.00 , 3.74)
(59.00 , 3.74)
(60.00 , 3.76)
(61.00 , 3.73)
(62.00 , 3.74)
(63.00 , 3.74)
(64.00 , 3.76)
(65.00 , 3.75)
(66.00 , 3.72)
(67.00 , 3.75)
(68.00 , 3.04)
(69.01 , 3.40)
(70.00 , 3.41)
(71.00 , 3.70)
(72.00 , 2.93)
(73.00 , 3.42)
(74.00 , 3.76)
(75.00 , 3.74)
(76.00 , 3.74)
(77.00 , 3.75)
(78.00 , 3.74)
(79.00 , 3.74)
(80.00 , 3.74)
(81.00 , 3.74)
(82.00 , 3.74)
(83.00 , 3.75)
(84.00 , 3.74)
(85.00 , 3.74)
(86.00 , 3.74)
(87.00 , 3.76)
(88.00 , 3.73)
(89.00 , 3.74)
(90.00 , 3.74)
(91.00 , 3.74)
(92.00 , 3.76)
(93.00 , 3.73)
(94.00 , 3.74)
(95.00 , 3.76)
(96.00 , 3.74)
(97.00 , 3.74)
(98.00 , 3.74)
(99.00 , 3.75)
(100.00 , 3.74)
(101.00 , 3.74)
(102.00 , 3.74)
(103.00 , 3.74)
(104.00 , 3.75)
(105.00 , 3.74)
(106.00 , 3.74)
(107.00 , 3.74)
(108.00 , 3.74)
(109.00 , 3.77)
(110.00 , 3.73)
(111.00 , 3.74)
(112.00 , 3.76)
(113.00 , 3.75)
(114.00 , 3.74)
(115.00 , 3.75)
(116.00 , 3.75)
(117.00 , 3.74)
(118.00 , 3.74)
(119.00 , 3.74)
(120.00 , 3.74) 

};\addlegendentry{Observed bandwidth}
\end{axis}
\end{tikzpicture}



==> figures/graphs/delay_graph_time.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[ybar, 
             ymax=200, 
             ymin=0,
             bar width=0.3,
             area style,
             xlabel={Time (s)},
	         ylabel={Delay (ms)},
	         legend style={at={(0.02,0.98)}, anchor=north west}]

\addplot[red] coordinates { 
(0.0649 , 52.2000)
(1.0652 , 18.0100)
(2.0673 , .0300)
(3.0696 , 40.8500)
(4.0703 , 87.2400)
(5.0708 , 83.4000)
(6.0709 , 129.2400)
(7.0727 , 91.1500)
(8.0747 , 63.6500)
(9.0759 , 19.3700)
(10.0784 , 56.9800)
(11.0806 , 61.9300)
(12.0811 , 42.0000)
(13.0822 , 30.5800)
(14.0846 , 85.9000)
(15.0861 , 48.3900)
(16.0882 , 100.3500)
(17.0912 , 117.1200)
(18.0950 , 57.0500)
(19.0953 , 27.5800)
(20.0976 , 46.0700)
(21.0995 , 12.3600)
(22.1013 , 45.3900)
(23.1024 , 81.6000)
(24.1028 , 23.0000)
(25.1050 , 41.0700)
(26.1061 , 100.4900)
(27.1077 , 37.1100)
(28.1079 , 63.6900)
(29.1103 , 45.7800)
(30.1138 , 96.2000)
(31.1158 , 38.5000)
(32.1180 , 34.6800)
(33.1190 , .0300)
(34.1214 , 15.6600)
(35.1239 , 41.6100)
(36.1256 , 126.0000)
(37.1289 , 60.6500)
(38.1294 , 13.9700)
(39.1309 , 66.4500)
(40.1330 , .0300)
(41.1364 , 27.1100)
(42.1383 , 85.8800)
(43.1395 , 48.9300)
(44.1407 , 32.0200)
(45.1426 , 23.9800)
(46.1444 , 59.0000)
(47.1468 , 62.0500)
(48.1480 , 93.5200)
(49.1487 , 32.0300)
(50.1506 , 26.6400)
(51.1525 , 115.6400)
(52.1559 , 39.1000)
(53.1590 , 45.9200)
(54.1598 , 51.0500)
(55.1613 , 75.9200)
(56.1614 , 19.1900)
(57.1615 , 59.7500)
(58.1615 , 73.8700)
(59.1619 , 35.6000)
(60.1623 , 120.6700)
(61.1643 , 92.6500)
(62.1645 , 41.1300)
(63.1649 , 12.7300)
(64.1659 , 40.3700)
(65.1670 , 104.0200)
(66.1690 , 50.7300)
(67.1694 , 26.6400)
(68.1707 , 4.0700)
(69.1738 , 20.0100)
(70.1753 , .0600)
(71.1782 , 22.0700)
(72.1804 , 83.5500)
(73.1816 , 83.4100)
(74.1833 , 71.5500)
(75.1836 , 58.4800)
(76.1856 , 69.2900)
(77.1861 , 50.9500)
(78.1876 , 83.7900)
(79.1882 , 86.7200)
(80.1886 , 6.0600)
(81.1916 , 51.8400)
(82.1925 , 32.9000)
(83.1938 , 76.1000)
(84.1943 , 139.5400)
(85.1966 , 158.6500)
(86.1992 , 70.1000)
(87.2005 , 73.5600)
(88.2017 , 57.5600)
(89.2035 , 69.5300)
(90.2043 , 48.8200)
(91.2052 , 24.7100)
(92.2077 , 61.4000)
(93.2085 , 29.3600)
(94.2099 , 12.5900)
(95.2120 , 66.6700)
(96.2125 , 95.0600)
(97.2129 , 12.3500)
(98.2157 , 65.2800)
(99.2162 , 66.7800)
};\addlegendentry{Observed Delay}


\end{axis}
\end{tikzpicture}


==> figures/traffic_generation.tex <==
\begin{table*}[!ht]
\centering
\begin{center}

% A table with adjusted row and column spacings
% \setlength sets the horizontal (column) spacing
% \arraystretch sets the vertical (row) spacing
\begingroup
\setlength{\tabcolsep}{8pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
\setlength\doublerulesep{.1pt}

%\small
%\footnotesize
\scriptsize
\begin{tabular}{
| 
>{\raggedright\arraybackslash}p{2.5cm} |
>{\raggedright\arraybackslash}p{0.6cm}|
>{\raggedright\arraybackslash}p{1cm}|
>{\raggedright\arraybackslash}p{0.3cm}  |
>{\raggedright\arraybackslash}p{0.9cm}  |
>{\raggedright\arraybackslash}p{0.9cm}  |
>{\raggedright\arraybackslash}p{0.9cm}  |
>{\raggedright\arraybackslash}p{0.7cm}  |
>{\raggedright\arraybackslash}p{1.1cm}  |
>{\raggedright\arraybackslash}p{1.2cm}  |
} 

\hline

% license type  ( opensource, comercial )
% language ( c++, python, java ; OTCL)
% GUI  ( yes, no, limited)
% Emulation support (no; yes; limited support)
% Scalability ( small, medium, large)
% Portability ( small, medium, large)

% Dynamic Link Support
% Real Traffic Generation Support
% Formal Description (verification)


% \hline
\rowcolor{gray}
 Name & 
 Open Source &  %Open source
 Language & 
 GUI & 
 Emulation Support & 
 Scalability & 
 Portability  & 
 Dynamic Link & 
 Automatic Traffic Generation & 
 Formal Description
\\
%& \begin{tabular}{@{}c@{}}Form \\ Descr \end{tabular} \\

 \hline
 Ns-3\cite{ns-3} & \checkmark & C++/Python & x & x & +++ & x & \checkmark & x & x\\
 %\hline
 %Ns-4\cite{fan2017ns4}	& \checkmark  & C++/Python & x & x & +++ & x & \checkmark & x & x\\
 \hline
 Mininet\cite{mininet} & \checkmark  & Python & \checkmark & \checkmark & + & \checkmark & x & x & x\\
 \hline
 Containernet\cite{containernet} & \checkmark  & Python & \checkmark & \checkmark & ++ & \checkmark & x & x & x\\
 \hline 
 OMNet++\cite{omnet} & x & C++ & \checkmark & x & +++ & x & \checkmark & x & x\\ 
 \hline
 Emulab\cite{stoller2008large}& \checkmark & C & \checkmark &  \checkmark & + & \checkmark & x & x & x\\
 \hline
 OpenNet\cite{chan2014opennet} & \checkmark & C++ & \checkmark & x & +++ & x & \checkmark & x & x \\
 \hline
 vSDNEmul\cite{farias2019vsdnemul}& \checkmark & Python & x & \checkmark & ++ & \checkmark & x &x  & x\\
 \hline
 EstiNet\cite{wang2013estinet}& x & - & \checkmark & \checkmark & ++ & \checkmark & \checkmark & - & -\\
 \hline
 SDN Owl\cite{srisawai2018rapid} & \checkmark & Python & x & \checkmark & ++ &\checkmark & x & x &x\\
% \hline
% Mesh Linux Containers (MLC)\cite{6379145} & \checkmark & -  & x & \checkmark & x & x & x & x & x\\
% \hline
% CORE (Common open research emulator)\cite{ahrenholz2008core} & \checkmark & Python & \checkmark & \checkmark & + & \checkmark & \checkmark & x& x\\ 
% \hline
%Cloonix3\cite{neumann2008better}& \checkmark & C & \checkmark & \checkmark & + & x & x & x & x\\
% \hline
%  GNS3\cite{neumann2015book} & \checkmark & Python & \checkmark & \checkmark & - & x & x & x & x\\ 
 \hline
 NetEM\cite{hemminger2005network}& \checkmark & - & x & \checkmark & - & x & \checkmark & x & x\\
% \hline
%  WANem\cite{kalitay2011designing}  & \checkmark & - & \checkmark& \checkmark & + & \checkmark & x & x & x\\
% \hline
% NEMAN\cite{puvzar2005neman} & \checkmark & Python & \checkmark & \checkmark & ++ & \checkmark & \checkmark & x & x\\
% \hline
 %MiniWorld\cite{schmidt2017miniworld} & \checkmark & Python & x & \checkmark & + & \checkmark & x &  x & x\\
 \hline
 
% \hline
% Ns-1\cite{mccannens}  & 3\checkmark & + & - & +/-/\checkmark & \\ [0.5ex] 
% \hline
% Ns-2\cite{issariyakul2009introduction} & 545 & 778 & 7507 &  33 & 22\\
 % \hline
% BAMNE\cite{britos2015batman}   & \checkmark & + & - & +/-/\checkmark & \\
%  \hline
%  Netkit\cite{pizzonia2008netkit} 	  & \checkmark & + & - & +/-/\checkmark & \\
 %\hline
 %MobiREAL\cite{1521172}  & \checkmark & + & - & +/-/\checkmark & \\
% \hline
% JiST/SWANs\cite{Barr:2005:JEA:1060168.1060170} & \checkmark & + & - & +/-/\checkmark & \\
% \hline
% S3F/S3FNet\cite{jin2014parallel}& \checkmark & + & - & +/-/\checkmark & \\


\end{tabular}
\endgroup

\end{center}
\caption{Comparison of Software-based Network Testbeds}
%\caption{Comparison of Software-based Network simulators/emulators}
\label{tab:survey}
\end{table*}











































% https://www.google.com/search?q=emulators+comparison&tbm=isch&ved=2ahUKEwjH5sDZxLv1AhW5YvEDHdevA8oQ2-cCegQIABAA&oq=emulators+comparison&gs_lcp=CgNpbWcQAzIGCAAQChAYOgUIABCABDoHCCMQ7wMQJzoECAAQQzoGCAAQCBAeOgQIABAYULYJWKEzYNA1aAFwAHgAgAE1iAGnB5IBAjIymAEAoAEBqgELZ3dzLXdpei1pbWfAAQE&sclient=img&ei=FtLmYceDILnFxc8P19-O0Aw&bih=907&biw=1790&client=ubuntu&hs=rdY#imgrc=wz0gNsJ-IXgBDM&imgdii=FLKJFVSp084bwM
% https://christian-krupitzer.github.io/files/2020_SIMUTools_IoT%20Network%20Emulator.pdf
% https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.227.7329&rep=rep1&type=pdf
% https://d1wqtxts1xzle7.cloudfront.net/35482600/researchpaper_Detail-Comparison-of-Network-Simulators-with-cover-page-v2.pdf?Expires=1642518150&Signature=TyzZEW48G4TFgFjYdR4~jtyOVvShXMx8wYvVHH2aZM2VzHWjnVRWFpE1w5VFt23vyCvjelimzqEYwIlKeAJkKBNkZqtu7O3WH4z0ah1PpB~X1AUS8uYdpGDQMOwsz71C-FUtAq0hacK9SBPzx2KnCZ~kvu48PixnVD0XbJmsI0-nkVIKP3ANkEW~MJbHOJCC93tSdsWDgKzUE9amPCeWuS8YmLML5kwQnX2i7louR1Kf3DRG29kZORlxe7U96tfMgSxRO9l-oRqXlBMuRQ0ksm2JMSN4bHHZQ5Vx1lHOc2XAkEPB5ILMRrKE0tmpie2DVzZGXmn2tpNdo1Hjl4NeOA__&Key-Pair-Id=APKAJLOHF5GGSLRBV4ZA
% https://scholar.google.com/scholar?hl=en&as_sdt=0%2C5&q=Network+simulator+emulator+comparison&btnG=

% https://hal.archives-ouvertes.fr/hal-00739154/document

% https://www.google.com/url?sa=i&url=https%3A%2F%2Fwww.researchgate.net%2Ffigure%2FComparison-of-network-simulators-and-emulators-in-a-learning-context_tbl1_328591250&psig=AOvVaw1nlJ65yiiUdx8A_1fdYXT4&ust=1642603422818000&source=images&cd=vfe&ved=0CAsQjRxqFwoTCIi_p9_Eu_UCFQAAAAAdAAAAABB7

% http://article.sapub.org/10.5923.j.jwnc.20150501.03.html http://article.sapub.org/10.5923.j.jwnc.20150501.03.html

% OS. -> Open source (license type)
% Language
% Wireless Networks Support  -> WNS
% Mobile Networks Support  -> WNS
% SDN Support -> SDNS
% Emulates real networks Interfaces
% User-friendly Interface 


% type (simulator; Emulator) https://www.google.com/url?sa=i&url=https%3A%2F%2Fwww.researchgate.net%2Ffigure%2FComparison-table-of-the-different-SDN-simulators-emulators_tbl6_323372308&psig=AOvVaw1nlJ65yiiUdx8A_1fdYXT4&ust=1642603422818000&source=images&cd=vfe&ved=0CAsQjRxqFwoTCIi_p9_Eu_UCFQAAAAAdAAAAABB2

% # one  https://www.google.com/url?sa=i&url=https%3A%2F%2Fwww.researchgate.net%2Ffigure%2FComparison-of-Ad-Hoc-network-Simulators-36-37_tbl6_310516691&psig=AOvVaw1nlJ65yiiUdx8A_1fdYXT4&ust=1642603422818000&source=images&cd=vfe&ved=0CAsQjRxqFwoTCIi_p9_Eu_UCFQAAAAAdAAAAABBx



% license type  ( opensource, comercial )
% language ( c++, python, java ; OTCL)
% GUI  ( yes, no, limited)
% simulation technique ( discrete event, )
% Scalability ( small, medium, large)
% Ease of use (Hard ; easy)
% Emulation support (no; yes; limited support)
% Suported Operating system (GNU/Linux; FreeBSD; MacOS, Windosws, )




==> sections/celullarAtm.tex <==
Cellular Automatas (CAs) are discrete dynamic models based on finite state machines (FSMs) called cells. Each cell next state is determined by an updating transition function, or rule, which gives the new state of the cell according to its current state and the current state of its nearest neighbors.





Here, we have considered 2-dimensional 4-neighborhood x-state CAs, each cell can assume any of the states S e Z. The CA has periodic boundary, that is, the cells of the CA form a ring L = Z/nZ , where n the number of cells of the CA. The rule of the CA is represented by R: S3 -> S

==> sections/dama.tex <==
%all this probably won't make the paper if we are writing a magazine... 

%The Demand Assigned Multiple Access~(DAMA) is a resource allocation scheme. As its name suggests, the idea is to assign physical resources to nodes which need to transmit traffic, according to their demands. The physical resources are translated to bandwidth. In real settings, in order to assign a given bandwidth the DAMA module may assign certain time slots and frequencies to a particular node (station). We abstract from this physical level and consider that the bandwidth to physical resource assignation is done by a proper translation module. Therefore, we are interested in the logical view of the algorithm, i.e., only the bandwidth assignations and no deeper. 

We denote the bandwidth demand per link as $d(e)$, where $e$ is an edge in the network. We assume that the the nodes have their corresponding minimum passing bandwidth (CIR, for committed information rate), and correspondingly its maximum passing bandwidth (MIR, for maximal information rate); these are denoted similarly as $m(e)$ and $c(e)$ for the MIR and CIR of $e$, respectively. Additionally, there is an overall bandwidth constant that the DAMA cannot exceed; this constant is known as the cluster bandwidth and it relates to the carrying frequencies that can be allocated for a given zone. We assume that the cluster bandwidth is denoted as $B$ and applies to all edges in the network topology; if there are multiple clusters within the topology, a partition of the edges can be made and the individual sets can be used. Finally, we assume that the bandwidth assignation per link is given as a function $b(e)$. In Algorithm~\ref{algo:dama}, we showcase the DAMA algorithm. Note that, the DAMA behavior should be the same for all implementations up to step number 3, however, step 4 differs from implementation to implementation. In Algorithm~\ref{algo:dama}, we chose to \emph{equally} distribute the remaining resources, up to a chosen allocation unit. Nonetheless, note that, the choice could have been a first come first served or any other (including a proportional allocation, or any other optimality criterion).  

\input{figures/dama_algorithm}

Note that, Algorithm~\ref{algo:dama}, is quite efficient. Depending on its parameters, in the worst case it has a running time of $\mathcal{O}(E+B/u)$. If $u<<B$, then, this running time can be high. Nevertheless, for satellite communications the bandwidth is in the order or Mbps; even for $u=1$, the order of $B$ is manageable. This is important as normally the bandwidth allocation changes each $125ms$ for satellite communications, and thus, the allocation algorithm must be able to terminate under that time. Finally, note that DAMA is often used in satellite communications as it is a great fit for this type of traffic.


